Neural Transformation Learning for Deep Anomaly Detection Beyond Images

Data transformations (e.g. rotations, reflections, and cropping) play an important role in self-supervised learning. Typically, images are transformed into different views, and neural networks trained on tasks involving these views produce useful feature representations for downstream tasks, including anomaly detection. However, for anomaly detection beyond image data, it is often unclear which transformations to use. Here we present a simple end-to-end procedure for anomaly detection with learnable transformations. The key idea is to embed the transformed data into a semantic space such that the transformed data still resemble their untransformed form, while different transformations are easily distinguishable. Extensive experiments on time series demonstrate that our proposed method outperforms existing approaches in the one-vs.-rest setting and is competitive in the more challenging n-vs.-rest anomaly detection task. On tabular datasets from the medical and cyber-security domains, our method learns domain-specific transformations and detects anomalies more accurately than previous work.

==> discussion.tex <==
\section{discussion}
\begin{itemize}
    \item summary
    \item holistic view
    \item local learning. For now we learn transformations at the data level but it would be interesting to learn transformations for each level of the hierarchy.
\end{itemize}

==> tables/sad_results.tex <==
\iffalse
\begin{table}[t!]
	\caption{Average AUC with standard deviation for n-vs-all anomaly detection on spoken Arabic digits.}
	\label{tab:sad_n-vs-all}
	\centering
%	\vspace{-5pt}
	\resizebox{\linewidth}{!}{
	\begin{tabular}{l|ccccc}
        \hline
		     & $n=1$   & $n=3$   &$n=5$ &$n=7$   &$n=9$\\
		\hline
        OC-SVM & 95.3 &74.2 &65.5&61.0&60.2\\
        IF & 88.2 &65.4 &59.7&57.5&56.9\\
        LOF & 98.3 &96.1 &94.9&93.1&93.1\\
        \hline
        RNN & 81.5$\pm$0.4 &60.7$\pm$0.4 &55.7$\pm$0.3&54.3$\pm$0.4&53.0$\pm$0.1 \\
        Deep-SVDD & 86.0$\pm$0.1 & 65.9$\pm$0.6 &61.5$\pm$1.2&58.0$\pm$0.6&59.7$\pm$0.5 \\
        DAGMM & 80.9$\pm$1.2 &52.6$\pm$1.2 &51.8$\pm$0.3&50.8$\pm$0.4&49.3$\pm$0.8 \\
        GOAD & 94.7$\pm$0.1 &83.4$\pm$0.6 &77.3$\pm$0.2&72.8$\pm$0.2& 70.5$\pm$1.4\\
        fixed Ts ($k$=12) & 96.7$\pm$0.1 & 89.1$\pm$0.5 &82.4$\pm$0.4&77.1$\pm$0.2& 74.8$\pm$1.3 \\
                \hline
        Our ($k$=12) & 98.9$\pm$0.1 &95.7$\pm$0.1  &91.3$\pm$0.2 &88.4$\pm$0.1 &85.1$\pm$0.3 \\
                \hline
	\end{tabular}}
%		\vspace{-12pt}
\end{table}

\begin{table*}[t!]
	\caption{AUC with standard deviation for rest-vs-all anomaly detection on spoken arabic digits.}
	\label{tab:ts_rest-vs-all}
	\centering
%	\vspace{-5pt}
	\resizebox{\textwidth}{!}{
	\begin{tabular}{l|ccc|ccccc|c}
        \hline
		     & OC-SVM   & IF   &LOF &RNN &Deep-SVDD   &DAGMM &GOAD &fixed Ts ($k$=12) &Our ($k$=12)\\
		\hline
        class 0 & 40.1 & 29.6 & 92.5 &30.5$\pm$0.8&59.3$\pm$1.3& 36.1$\pm$2.7 &65.2$\pm$0.6 &50.8$\pm$1.3&89.8$\pm$0.2\\
        class 1 & 68.5 & 51.8 & 97.6 &36.6$\pm$0.3&61.7$\pm$3.8& 51.3$\pm$1.3 & 78.5$\pm$4.1&96.2$\pm$1.0 &98.5$\pm$0.1\\
        class 2 & 79.6 & 76.4 & 97.3 &67.9$\pm$0.5&57.7$\pm$8.4& 63.3$\pm$4.7 & 89.1$\pm$1.1 &93.9$\pm$0.6&89.1$\pm$0.3\\
        class 3 & 65.0 & 76.1 & 98.5 &74.1$\pm$0.3&65.7$\pm$3.4& 34.4$\pm$0.2 & 74.6$\pm$5.8 &77.2$\pm$6.5&91.1$\pm$0.3\\
        class 4 & 51.3 & 52.2 & 87.2 &60.9$\pm$0.5&46.9$\pm$2.4& 51.2$\pm$1.4 & 63.6$\pm$2.7 &79.1$\pm$0.2&77.6$\pm$0.4\\
        class 5 & 59.3 & 38.9 & 97.7 &31.1$\pm$0.5&65.2$\pm$0.6& 55.0$\pm$2.6 & 88.0$\pm$0.8 &93.3$\pm$1.4&97.0$\pm$0.1\\
        class 6 & 93.6 & 82.4 & 85.5 &78.0$\pm$0.5&86.0$\pm$2.9& 60.9$\pm$0.2 & 77.5$\pm$1.0 &67.5$\pm$0.9&77.1$\pm$0.8\\
        class 7 & 47.8 & 38.6 & 84.9 &38.1$\pm$0.5&44.2$\pm$0.4& 52.0$\pm$2.1 & 51.6$\pm$1.5 &40.3$\pm$1.9&68.4$\pm$1.1\\
        class 8 & 47.7 & 87.0 & 98.4 &85.8$\pm$0.2&60.9$\pm$7.8& 53.8$\pm$3.8 & 58.9$\pm$3.8 &81.8$\pm$3.5&98.3$\pm$0.1\\
        class 9 & 49.1 & 35.7 & 91.9 &26.6$\pm$0.2&49.2$\pm$0.5& 34.9$\pm$1.1 & 56.8$\pm$2.6 &68.4$\pm$2.9&63.6$\pm$2.7\\
        \hline
        Average & 60.2 & 56.9 & 93.1 &53.0$\pm$0.1&59.7$\pm$0.5& 49.3$\pm$0.8 & 70.5$\pm$1.4 &74.8$\pm$1.3&85.1$\pm$0.3\\
        \hline
	\end{tabular}}
%		\vspace{-12pt}
\end{table*}
\fi
